FlashDecoding++: Faster Large Language Model Inference on GPUs

As the Large Language Model (LLM) becomes increasingly important in various domains. However, the following challenges still remain unsolved in accelerating LLM inference: (1) Synchronized partial softmax update. The softmax operation requires a synchronized update operation among each partial softmax result, leading to ~20% overheads for the attention computation in LLMs. (2) Under-utilized computation of flat GEMM. The shape of matrices performing GEMM in LLM inference is flat, leading to under-utilized computation and >50% performance loss after padding zeros in previous designs. (3) Performance loss due to static dataflow. Kernel performance in LLM depends on varied input data features, hardware configurations, etc. A single and static dataflow may lead to a 50.25% performance loss for GEMMs of different shapes in LLM inference. We present FlashDecoding++, a fast LLM inference engine supporting mainstream LLMs and hardware back-ends. To tackle the above challenges, FlashDecoding++ creatively proposes: (1) Asynchronized softmax with unified max value. FlashDecoding++ introduces a unified max value technique for different partial softmax computations to avoid synchronization. (2) Flat GEMM optimization with double buffering. FlashDecoding++ points out that flat GEMMs with different shapes face varied bottlenecks. Then, techniques like double buffering are introduced. (3) Heuristic dataflow with hardware resource adaptation. FlashDecoding++ heuristically optimizes dataflow using different hardware resource considering input dynamics. Due to the versatility of optimizations in FlashDecoding++, FlashDecoding++ can achieve up to 4.86x and 2.18x speedup on both NVIDIA and AMD GPUs compared to Hugging Face implementations. FlashDecoding++ also achieves an average speedup of 1.37x compared to state-of-the-art LLM inference engines on mainstream LLMs.

==> tex/AMD_impl.tex <==
\section{Implementation on AMD} \label{appendix_AMD}
%
Due to the PyTorch's support for AMD GPUs, we can perform large language model inference on AMD GPUs similar to what we do on NVIDIA GPUs. 
We have implemented and validated the effectiveness of our proposed methods on AMD GPUs using AMD parallel programming.
AMD parallel programming shares many similarities with NVIDIA parallel programming. 
Their programming models are divided into grid, block, warp, and thread. 
Similar to the CUDA runtime library of NVIDIA, AMD has the ROCm runtime library. 
We can use HIP to develop kernels for AMD GPUs. 
HIP has APIs that closely resemble CUDA APIs.
We can easily port CUDA code developed for NVIDIA GPUs to HIP code for AMD GPUs by modifying the API names or using the HIPIFY tool \cite{hipify}. 
However, architectural differences between GPUs mean that efficient kernels developed for NVIDIA GPUs may not necessarily be efficient on AMD GPUs, and in some cases, they may not even run. 
For example, consumer-level GPU like the RX7900XTX, based on the RDNA3 architecture, lacks structures similar to the Tensor Core and cannot efficiently perform matrix operations using WMMA instructions as CUDA. 
In contrast, compute-level GPU like the MI210, based on the CDNA2 architecture, has the Matrix Core but with a warp size of 64, unlike NVIDIA GPUs. 
This necessitates optimizations tailored for each of these GPUs.

We employ different strategies for our implementations on these two types of AMD GPUs to accommodate their distinct characteristics compared to NVIDIA GPUs. 
Since our asynchronized softmax optimization does not use the Tensor Core, we migrate CUDA codes to HIP and run them on these two types of AMD GPUs. 
However, the flat GEMM optimization uses the Tensor Core, so we need different implementation approaches for the RX7900XTX and MI210. 
Given that MI210 has Matrix Cores, a hardware structure similar to Tensor Cores for efficient matrix computation, we migrate CUDA code and adjust the warp size to 64 to suit this GPU. 
RX7900XTX does not have Matrix Cores, preventing direct code migration. To this end, we use the WMMA compiler intrinsics, such as \texttt{\_\_builtin\_amdgcn\_wmma\_f16\_16x16x16\_f16\_w32}, to develop flat GEMM kernels resulting in $20\%$ speedup than the torch.matmul used in PyTorch on the RX7900XTX.
